Safety Challenges for Autonomous Vehicles in the Absence of Connectivity

Autonomous vehicles (AVs) are promoted as a technology that will create a future with effortless driving and virtually no traffic accidents. AV companies claim that, when fully developed, the technology will eliminate 94% of all accidents that are caused by human error. These AVs will likely avoid the large number of crashes caused by impaired, distracted or reckless drivers. But there remains a significant proportion of crashes for which no driver is directly responsible. In particular, the absence of connectivity of an AV with its neighboring vehicles (V2V) and the infrastructure (I2V) leads to a lack of information that can induce such crashes. Since AV designs today do not require such connectivity, these crashes would persist in the future. Using prototypical examples motivated by the NHTSA pre-crash scenario typology, we show that fully autonomous vehicles cannot guarantee safety in the absence of connectivity. Combining theoretical models and empirical data, we also argue that such hazardous scenarios will occur with a significantly high probability. This suggests that incorporating connectivity is an essential step on the path towards safe AV technology.

==> abstract.tex <==
%auto-ignore
\section*{Abstract}
Autonomous vehicles (AVs)  are promoted as a  technology that will create a future with effortless driving  and virtually no traffic accidents.
 AV companies claim that, when fully developed,  the technology will eliminate 94\% of all accidents that are caused by human error. These AVs will likely avoid the large number of crashes caused by impaired, distracted or reckless drivers. But there remains a significant proportion of crashes for which no driver is directly responsible. In particular, the absence of connectivity of an AV with its neighboring vehicles (V2V) and the infrastructure (I2V) leads to a lack of information that can induce  such crashes. Since  AV designs today do not require such connectivity,  these crashes would persist in the future. Using prototypical examples motivated by the NHTSA pre-crash scenario typology, we show that fully autonomous vehicles cannot guarantee safety in the absence of connectivity. Combining theoretical models and empirical data, we also argue that such hazardous scenarios will occur with a significantly high probability. This suggests that incorporating connectivity is an essential step on the path towards  safe AV technology.


==> format.tex <==
%auto-ignore


%\IEEEoverridecommandlockouts
%\overrideIEEEmargins
\usepackage{epsfig}
%\usepackage{subfigure}
\usepackage{amssymb,amsmath,amsfonts,layout,graphicx}
\usepackage{makeidx}
\usepackage[english]{babel}
\usepackage{tikz}
\usepackage{sublabel}
\usepackage{cases}
\usepackage{algorithm}
\usepackage{algorithmic}

\usepackage{xcolor}

%\pagestyle{plain}
%\makeatletter
%
%\theoremstyle{plain}
%\newtheorem{definition}{\protect\definitionname}
%\newtheorem{problem}{\protect\problemname}
%\newtheorem{lemma}{\protect\lemmaname}
%\newtheorem{assumption}{\protect\assumptionname}
%\newtheorem{proposition}{\protect\propositionname}
%\newtheorem{theorem}{\protect\theoremname}


\setlength\parindent{0in}
\setlength\parskip{0.12in}

%\usepackage{vmargin}
%\setpapersize{USletter}
%\setmarginsrb{19.1mm}{19.1mm}{19.1mm}{19.1mm}{0pt}{0pt}{0pt}{0pt}
%\makeatother
\usepackage
[
        letterpaper,% other options: a3paper, a5paper, etc
        left=1.91cm,
        right=1.91cm,
        top=1.91cm,
        bottom=2cm,
        % use vmargin=2cm to make vertical margins equal to 2cm.
        % us  hmargin=3cm to make horizontal margins equal to 3cm.
        % use margin=3cm to make all margins  equal to 3cm.
]
{geometry}
\providecommand{\definitionname}{Definition}
\providecommand{\problemname}{Problem}
\providecommand{\lemmaname}{Lemma}
\providecommand{\assumptionname}{Assumption}
\providecommand{\propositionname}{Proposition}
\providecommand{\theoremname}{Theorem}
\providecommand{\examplename}{Example}

\setlength\parindent{0in}
\setlength\parskip{0.12in}

%\theoremstyle{plain}
\newtheorem{problem}{Problem}
\newtheorem{implication}{Implication}

\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}

% \newcommand{\R}{{\mathbb R}}
% \newcommand{\C}{{\mathbb C}}
% \newcommand{\N}{{\mathbb N}}
% \newcommand{\M}{{\mathbb M}}
% \newcommand{\Z}{{\mathbb Z}}


% \newcommand{\s}{\mathscr}
% \newcommand{\x}{{\bf x}}
% \newcommand{\q}{{\bf q}}
% \newcommand{\U}{{\bf U}}
% \renewcommand{\u}{{\bf u}}
% \newcommand{\X}{{\bf X}}
% \newcommand{\Q}{{\bf Q}}
% \renewcommand{\labelenumi}{(\roman{enumi})}
% \renewcommand{\th}{{\text{th}}}
